Correlated Source Coded Sequences with Compromised Channel and Source Symbols using Shannon's Cipher System

Correlated sources are present in communication systems where protocols ensure that there is some predetermined information for sources to transmit. Here, two correlated sources across a channel with eavesdroppers are investigated, and conditions for perfect secrecy when some channel information and some source data symbols (the predetermined information) have been wiretapped are determined. The adversary in this situation has access to more information than if a link is wiretapped only and can thus determine more about a particular source. This scenario caters for an application where the eavesdropper has access to some preexisting information. We provide bounds for the channel and key rates for this scenario. Further, we provide a method to reduce the key lengths required for perfect secrecy.

==> bib.tex <==
\begin{document}


\begin{bib}{99}



@InProceedings{active_eavesdropper_aggarwal,
author = {V Aggarwal and L Lai and A.R Calderbank and H.V Poor},
title = {{W}iretap {C}hannel {T}ype II with an {A}ctive {E}avesdropper},
booktitle = {IEEE International Symposium on Information Theory},
OPTcrossref = {•},
OPTkey = {•},
pages = {1944 - 1948},
year = {2008},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
month = {June},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}


@InProceedings{side_information_dai,
author = {B Dai, Y Luo, A.J.H Vinck},
title = {{W}iretap {C}hannel with {S}ide {I}nformation from {P}art of {E}ncoder},
booktitle = {IFIP International Conference on Network and Parallel Computing},
OPTcrossref = {•},
OPTkey = {•},
pages = {353 - 357},
year = {2008},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}



@Article{gaussian_wiretap_mitrpant,
author = {C Mitrpant and A.J.H Vinck and Y Luo},
title = {{A}n {A}chievable {R}egion for the {G}aussian {W}iretap {C}hannel {W}ith {S}ide {I}nformation},
journal = {IEEE Transactions on Information Theory},
year = {2006},
OPTkey = {•},
volume = {52},
number = {5},
pages = {•},
month = {May},
OPTnote = {•},
OPTannote = {•}
}



@Article{shannon_secrecy_merhav,
author = {N Merhav},
title = {{S}hannon’s {S}ecrecy {S}ystem {W}ith {I}nformed {R}eceivers and its {A}pplication to {S}ystematic {C}oding for {W}iretapped {C}hannels
},
journal = {IEEE Transactions of Information Theory},
year = {2008},
OPTkey = {•},
volume = {54},
number = {6},
pages = {2723 - 2734},
month = {June},
OPTnote = {•},
OPTannote = {•}
}


@InProceedings{arxiv1_bal_ling,
author = {R Balmahoon and L Cheng},
title = {{I}nformation {L}eakage of {C}orrelated {S}ource {C}oded
{S}equences over {W}iretap {C}hannel},
booktitle = {arXiv},
OPTcrossref = {•},
OPTkey = {•},
pages = {1 - 20},
year = {2014},
OPTeditor = {},
OPTvolume = {•},
number = {1401.6264},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}



@Article{pablo_secure_multiterminal,
author = {J Villard and P Piantanida},
title = {{S}ecure {M}ultiterminal {S}ource {C}oding {W}ith {S}ide {I}nformation at the {E}avesdropper},
journal = {IEEE Transactions on Information Theory},
year = {2013},
OPTkey = {•},
volume = {59},
number = {6},
pages = {3668 - 3692},
month = {June},
OPTnote = {•},
OPTannote = {•}
}

@Article{pablo_secure_transmission_receivers,
author = {J Villard, P Piantanida and S Shamai},
title = {{S}ecure {T}ransmission of {S}ources {O}ver {N}oisy {C}hannels {W}ith {S}ide {I}nformation at the {R}eceivers},
journal = {IEEE Transactions of Information Thory},
year = {2014},
OPTkey = {•},
volume = {60},
number = {1},
pages = {713 - 739},
month = {January},
OPTnote = {•},
OPTannote = {•}
}


@InProceedings{pablo_hybrid,
author = {•},
title = {Hybrid {D}igital/{A}nalog {S}chemes for {S}ecure {T}ransmission with {S}ide {I}nformation},
booktitle = {IEEE Information Theory Workshop},
OPTcrossref = {•},
OPTkey = {•},
pages = {678 - 682},
year = {2011},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}


@Book{yeung_course,
ALTauthor = {R.W Yeung},
OPTALTeditor = {•},
title = {A first course in Information Theory},
publisher = {Kluwer Academic/Plenum Publishers},
year = {2002},
OPTkey = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTedition = {•},
OPTmonth = {•},
OPTnote = {•},
OPTannote = {•}
}


 @Article{coding_yamamoto,
 author = {H Yamamoto},
 title = {Coding Theorem for Secret Sharing Communication Systems with Two Noisy Channels},
 journal = {IEEE Transactions on Information Theory},
 year = {1989},
 OPTkey = {•},
 volume = {35},
 number = {3},
 pages = {572 - 578},
 month = {May},
 OPTnote = {•},
 OPTannote = {•}
 }


 @Article{shannon1_yamamoto,
 author = {H Yamamoto},
 title = {Coding Theorems for Shannon's Cipher System with Correlated Source Ouputs, and Common Information},
 journal = {IEEE Transactions on Information Theory},
 year = {1994},
 OPTkey = {•},
 volume = {40},
 number = {1},
 pages = {85 - 95},
 month = {January},
 OPTnote = {•},
 OPTannote = {•}
 }
 
 @Article{hayashi_yamamoto,
 author = {Hayashi K and Yamamoto H},
 title = {Coding Theorems for the Shannon Cipher System With a Guessing Wiretapper and Correlated Source Outputs},
 journal = {IEEE Transactions on Information Theory},
 year = {2008},
 OPTkey = {•},
 volume = {54},
 number = {6},
 pages = {2808 - 2817},
 month = {June},
 OPTnote = {•},
 OPTannote = {•}
 }
 \begin{document}


\begin{bibli1}{99}


@InProceedings{ ref1_del_landi,
author = {PG Del and C Landi},
title = {Real-time smart meter with embedded web server capability},
booktitle = {IEEE International Conference on Instrumentation and Measurement Technology},
pages = {682 - 687},
year = {2012},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}

@Article{ ref2_xia_wang,
author = {J Xia and Y Wang},
title = {Secure Key Distribution for the Smart Grid},
journal = {IEEE Transactions on Smart Grid},
year = {2012},
OPTkey = {•},
volume = {3},
number = {3},
pages = {1437 - 1443},
month = {September},
OPTnote = {•},
OPTannote = {•}
}

@InProceedings{ ref3_moslehi_kumar,
author = {K Moslehi and R Kumar},
title = {Smart Grid - a reliability perspective},
booktitle = {Conference on Innovative Smart Grid Technologies (ISGT)},
OPTcrossref = {•},
OPTkey = {•},
pages = {1 - 8},
year = {2010},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}

@Article{ ref4_lo_ansari,
author = {C Lo and N Ansari},
title = {The Progressive Smart Grid System from Both Power and Communications Aspects},
journal = {IEEE Communications Surveys and Tutorials},
year = {2012},
OPTkey = {•},
volume = {14},
number = {3},
pages = {799 - 819},
month = {Third Quarter},
OPTnote = {•},
OPTannote = {•}
}

@InProceedings{ ref5_huang_hu,
author = {J Huang and X Hu and L Li and H Ketai},
title = {Design of New Architecture of AMR System in Smart Grid},
booktitle = {IEEE Conference on Industrial Electronics and Applications (ICIEA)},
OPTcrossref = {•},
OPTkey = {•},
pages = {2025 - 2029},
year = {2011},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}

@InProceedings{ ref6_wang_li,
author = {X Wang and W Li},
title = {The Research of AMR in Smart Meter},
booktitle = {Asia-Pacific Power and Energy Engineering Conference (APPEEC)},
OPTcrossref = {•},
OPTkey = {•},
pages = {1 - 4},
year = {2010},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}

@InProceedings{ ref7_he_jagmohan,
author = {D He and A Jagmohan and L Ligang},
title = {Secure collaboration using Slepian-Wolf codes},
booktitle = {15th IEEE International Conference on Image Processing},
OPTcrossref = {•},
OPTkey = {•},
pages = {2216 - 2219},
year = {2008},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}

@article{ref8_kurkoski_wolf,
  title={Slepian-Wolf coding},
  author={Wolf, Jack K and Kurkoski, Brian M},
  journal={Scholarpedia},
  volume={3},
  number={11},
  pages={6789},
  year={2008}
}

@Article{ ref9_slepian_wolf,
author = {D Slepian and J.K Wolf},
title = {Noiseless Coding of Correlated Information Sources},
journal = {IEEE Transactions on Information Theory},
year = {1973},
OPTkey = {•},
volume = {19},
number = {4},
pages = {471 - 480},
month = {July},
OPTnote = {•},
OPTannote = {•}
}

@InProceedings{ ref10_stankovic_liveris,
author = {V Stankovic and A.D Liveris and Z Xiong and C.N Georghiades},
title = {Design of Slepian Wolf Codes by Channel Code Partitioning},
booktitle = {IEEE Data Compression Conference},
OPTcrossref = {•},
OPTkey = {•},
pages = {302 - 311},
year = {2004},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}

@Article{ ref11_cai_yeung,
author = {N Cai and R.W Yeung},
title = {Secure Network Coding on a Wiretap Network},
journal = {IEEE Transactions on Information Theory,},
year = {2011},
OPTkey = {•},
volume = {57},
number = {1},
pages = {424 - 435},
month = {January},
OPTnote = {•},
OPTannote = {•}
}

@Article{ ref12_rouayheb_soljanin,
author = {S.E Rouayheb and Soljanin E and A Sprintson},
title = {Secure Network Coding for Wiretap Networks of Type II},
journal = {IEEE Transactions on Information Theory},
year = {2012},
OPTkey = {•},
volume = {58},
number = {3},
pages = {1361 - 1371},
month = {March},
OPTnote = {•},
OPTannote = {•}
}

@Article{ ref13_wei,
author = {V.K Wei},
title = {Generalized Hamming Weights for Linear Codes},
journal = {IEEE Transactions on Information Theory,},
year = {1991},
OPTkey = {•},
volume = {37},
number = {5},
pages = {1412 - 1418},
month = {September},
OPTnote = {•},
OPTannote = {•}
}

@Article{ ref14_luo_mitpant,
author = {Y Luo and C Mitpant and A.J.H Vinck},
title = {Some New Characteristics on the Wiretap Channel of Type II},
journal = {IEEE Transactions on Information Theory},
year = {2005},
OPTkey = {•},
volume = {51},
number = {3},
pages = {1222 - 1229},
month = {March},
OPTnote = {•},
OPTannote = {•}
}

@InProceedings{ ref15_ozarow_wyner,
author = {L.H Ozarow and A.D Wyner},
title = {Wire-Tap Channel II},
booktitle = {Advances in Cryptology - EUROCRYPT},
OPTcrossref = {•},
OPTkey = {•},
pages = {33 - 50},
year = {1985},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}

@InProceedings{ ref16_ho_medard,
author = {T Ho and M Médard and M Effros and R Koetter},
title = {Network Coding for Correlated Sources},
booktitle = {Proceedings of Conference for Information Science and Systems},
OPTcrossref = {•},
OPTkey = {•},
pages = {1 - 6},
year = {2004},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}


@InProceedings{ ref17_buyukalp_maatouk,
author = {Y Buyukalp and G Maatouk and V.M Prabhakaran and C Fragouli},
title = {Untrusting Network Coding},
booktitle = {International Symposium on Network Coding},
OPTcrossref = {•},
OPTkey = {•},
pages = {79 - 84},
year = {2012},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}

@InProceedings{ref18_luo_dimakis,
author = {J Luo and A. G Dimakis and D.S Papailiopoulos  and C Huang and Jin Li},
title = {Simple Regenerating Codes: Network Coding for Cloud Storage},
booktitle = {International Conference on Computer Communications},
OPTcrossref = {•},
OPTkey = {•},
pages = {2801 - 2805},
year = {2012},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}


@Article{ref19_ho_leong,
author = {T Ho and B Leong and R Koetter and M Medard and M Effros and D.R Karger},
title = {Byzantine Modification Detection in Multicast Networks with Random Network Coding},
journal = {IEEE Transactions on Information Theory},
year = {2008},
OPTkey = {•},
volume = {54},
number = {6},
pages = {2798 - 2803},
month = {June},
OPTnote = {•},
OPTannote = {•}
}

@Article{ref20_yeung_zhang,
author = {R.W Yeung and Z Zhang},
title = {Distributed Source Coding for Satellite Communications},
journal = {IEEE Transactions on Information Theory},
year = {1999},
OPTkey = {•},
volume = {45},
number = {4},
pages = {1111 - 1120},
month = {May},
OPTnote = {•},
OPTannote = {•}
}

@InProceedings{ref21_cheng_yeung,
author = {F Cheng and R.W Yeung and K.W Shum},
title = {Imperfect Secrecy in Wiretap Channel II},
booktitle = {IEEE International Symposium on Information Theory},
OPTcrossref = {•},
OPTkey = {•},
pages = {71 - 75},
year = {2012},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}

@InProceedings{ref22_chi_cheng,
author = {W Chi and H Cheng and H Xiaotao},
title = {A Combination Scheme against Pollution Attacks in Network Coding},
booktitle = {IEEE 11th Internation Conference on Computer and Information Science},
OPTcrossref = {•},
OPTkey = {•},
pages = {71 - 76},
year = {2012},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}

@InProceedings{vinck_biometrics,
author = {A.J.H Vinck},
title = {Applications of Coding and Information Theory in Biometrics},
booktitle = {19th European Signal Processsing Conference},
OPTcrossref = {•},
OPTkey = {•},
pages = {2254 - 2258},
year = {2011},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
month = {August},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}

@InProceedings{nc_wiretap_capar,
author = {C.Capar and D. Goeckel},
title = {Network coding for facilitating secrecy in large wireless networks },
booktitle = {Conference on Information Sciences and Systems},
OPTcrossref = {•},
OPTkey = {•},
pages = {1 - 6},
year = {2012},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}

@InProceedings{info_leakage_sun,
author = {W Sun and S Rane},
title = {On Information Leakage During Secure Verification of Compatibility Between Signals},
booktitle = {Canadian Workshop on Information Theory},
OPTcrossref = {•},
OPTkey = {•},
pages = {75 - 78},
year = {2009},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
month = {June},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}

@InProceedings{biomentrics_draper,
author = {S.C Draper and A Khisti and E Martinian and A Vetro},
title = {Secure storage of fingerprint biometrics using Slepian-Wolf codes},
booktitle = {Information Theory and Apps. Workshop, UCSD},
OPTcrossref = {•},
OPTkey = {•},
OPTpages = {•},
year = {2007},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
OPTmonth = {•},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}

@Article{client_server_bloch,
 author = {M Bloch and R Narasimha and S.W McLaughlin},
 title = {Network Security for Client-Server Architecture Using Wiretap Codes},
 journal = {IEEE Transactions on Information Forensics and Security},
 year = {2008},
 OPTkey = {•},
 volume = {3},
 number = {3},
 pages = {404 - 413},
 month = {September},
 OPTnote = {•},
 OPTannote = {•}
 }
  
 @Article{hamming_ngai,
 author = {C Ngai and R.W Yeung and Z Zhang},
 title = {Network Generalized Hamming Weight},
 journal = {IEEE Transactions on Information Theory},
 year = {2011},
 OPTkey = {•},
 volume = {57},
 number = {2},
 pages = {1136 - 1143},
 month = {February},
 OPTnote = {•},
 OPTannote = {•}
 }
 
 @InProceedings{source_coding_grokop,
 author = {L Grokop and A Sahai and M Gastpar},
 title = {Discriminatory Source Coding for a Noiseless Broadcast Channel},
 booktitle = {International Syposium on Infomation Theory},
 OPTcrossref = {•},
 OPTkey = {•},
 pages = {77 - 81},
 year = {2005},
 OPTeditor = {•},
 OPTvolume = {•},
 OPTnumber = {•},
 OPTseries = {•},
 OPTaddress = {•},
 OPTmonth = {•},
 OPTorganization = {•},
 OPTpublisher = {•},
 OPTnote = {•},
 OPTannote = {•}
 }
 
 
 @InProceedings{rank_metric_silva,
 author = {D Silva and R Kschischang},
 title = {Security for Wiretap Networks via Rank-Metric Codes},
 booktitle = {IEEE International Symposium on Information Theory},
 OPTcrossref = {•},
 OPTkey = {•},
 pages = {176 - 180},
 year = {2008},
 OPTeditor = {•},
 OPTvolume = {•},
 OPTnumber = {•},
 OPTseries = {•},
 OPTaddress = {•},
 month = {July},
 OPTorganization = {•},
 OPTpublisher = {•},
 OPTnote = {•},
 OPTannote = {•}
 }
 
 @Article{feedback_yang,
 author = {E Yang and D He and T  Uyematsu and R.W Yeung},
 title = {Universal {M}ultiterminal {S}ource {C}oding {A}lgorithms with {A}symptotically {Z}ero {F}eedback: {F}ixed {D}atabase {C}ase},
 journal = {IEEE Transactions on Information Theory},
 year = {2008},
 OPTkey = {•},
 volume = {54},
 number = {12},
 pages = {5575 - 5590},
 month = {December},
 OPTnote = {•},
 OPTannote = {•}
 }
 
 @Article{shannon1_yamamoto,
 author = {H Yamamoto},
 title = {Coding Theorems for Shannon's Cipher System with Correlated Source Ouputs, and Common Information},
 journal = {IEEE Transactions on Information THeory},
 year = {1994},
 OPTkey = {•},
 volume = {40},
 number = {1},
 pages = {85 - 95},
 month = {January},
 OPTnote = {•},
 OPTannote = {•}
 }
 
 @Article{shannon2_yamamoto,
 author = {H Yamamoto},
 title = {Rate-Distortion Theory for the Shannon Cipher System},
 journal = {IEEE Transactions on Information Theory},
 year = {1997},
 OPTkey = {•},
 volume = {43},
 number = {3},
 pages = {827 - 835},
 month = {May},
 OPTnote = {•},
 OPTannote = {•}
 }
 
 @Article{coding_yamamoto,
 author = {H Yamamoto},
 title = {Coding Theorem for Secret Sharing Communication Systems with Two Noisy Channels},
 journal = {IEEE Transactions on Information Theory},
 year = {1989},
 OPTkey = {•},
 volume = {35},
 number = {3},
 pages = {572 - 578},
 month = {May},
 OPTnote = {•},
 OPTannote = {•}
 }


 @Article{msc_thesis_26,
 author = {G Mark and N.M Su},
 title = {Making infrastructure visible for nomadic work},
 journal = {Pervasive and Mobile Computing},
 year = {2010},
 OPTkey = {•},
 OPTvolume = {•},
 OPTnumber = {•},
 pages = {312 - 323},
 OPTmonth = {•},
 OPTnote = {•},
 OPTannote = {•}
 
 @Article{msc_thesis_27,
 author = {J Hoebeke and I Moerman and B Dhoedt and P Demeester},
 title = {An Overview of Mobile Ad Hoc Networks: Applications and Challenges},
 journal = {Ghent University, Belgium, Department of Information Technology},
 OPTyear = {•},
 OPTkey = {•},
 OPTvolume = {•},
 OPTnumber = {•},
 pages = {60 - 66},
 OPTmonth = {•},
 OPTnote = {•},
 OPTannote = {•}
 } 
 
@Book{msc_thesis_33,
      author = {A Goldsmith},
      ALTeditor = {•},
      title = {Wireless Communications},
      publisher = {Cambridge University Press},
      year = {2005},
      OPTkey = {•},
      OPTvolume = {•},
      OPTnumber = {•},
      OPTseries = {•},
      address = {United States of America},
      edition = {1},
      OPTmonth = {•},
      OPTnote = {•},
      OPTannote = {•}
      }
            
            
@Article{foutain_byers_luby,
author = {J.W Byers; M Luby; M Mitzenmacher},
title = {A digital fountain approach to asynchronous reliable multicast},
journal = {IEEE Journal on Selected Areas in Communications},
year = {2002},
OPTkey = {•},
volume = {20},
number = {8},
pages = {1528 - 1540},
month = {October},
OPTnote = {•},
OPTannote = {•}
}


@InProceedings{zhang_partial_leakage,
author = {Z Zhang},
title = {Wiretap networks II with partial information leakage},
booktitle = {Fourth International Conference on Communications and Networking (ChinaCOM)},
OPTcrossref = {•},
OPTkey = {•},
pages = {1 - 5},
year = {2009},
OPTeditor = {•},
OPTvolume = {•},
OPTnumber = {•},
OPTseries = {•},
OPTaddress = {•},
month = {August},
OPTorganization = {•},
OPTpublisher = {•},
OPTnote = {•},
OPTannote = {•}
}



       
\end{bibli1}

\end{document}


\end{bib}
\end{document}
